"A Posteriori" Limited High Order and Robust Residual Distribution Schemes for Transient Simulations of Fluid Flows in Gas Dynamics

In this paper, we propose a novel approximation strategy for time-dependent hyperbolic systems of conservation laws for the Euler system of gas dynamics that aims to represent the dynamics of strong interacting discontinuities. The goal of our method is to allow an approximation with a high-order of accuracy in smooth regions of the flow, while ensuring robustness and a non-oscillatory behaviour in the regions of steep gradients, in particular across shocks. Following the Multidimensional Optimal Order Detection (MOOD) (Clain et al., Journal of Computational Physics 2011; Diot et al., Computer & Fluids 2012) approach, a candidate solution is computed at a next time level via a high-order accurate explicit scheme (Abgrall, Journal of Scientific Computing 2017; Abgrall et al., Computers & Mathematics with Applications 2018). A so-called detector determines if the candidate solution reveals any spurious oscillations or numerical issue and, if so, only the troubled cells are locally recomputed via a more dissipative scheme. This allows to design a family of "a posteriori" limited, robust and positivity preserving, as well as high accurate, non-oscillatory and effective scheme. Among the detecting criteria of the novel MOOD strategy, two different approaches from literature, based on the work of Clain et al. (Journal of Computational Physics 2011), Diot et al. (Computer & Fluids 2012) and of Vilar (Journal of Computational Physics 2019), are investigated. Numerical examples in 1D and 2D, on structured and unstructured meshes, are proposed to assess the effective order of accuracy for smooth flows, the non-oscillatory behaviour on shocked flows, the robustness and positivity preservation on more extreme flows.

==> frame.tex <==
%
%  E U L E R     E Q U A T I O N S
%
\section{Hydrodynamics system of conservation laws}
\label{sec:Euler}
The model considered in this paper is the Euler system of equations for compressible gasdynamics in two space dimensions that reads, recalling Section \ref{EulerSystem_Preliminary_Section} for the reader's ease:
\begin{equation}
\label{system_hyp_mood}
 \frac{\partial}{\partial t} \left( \begin{array}{c} \rho \\ \rho \mathbf{u} \\  E \end{array} \right) +
 \nabla \cdot \left( 
 \begin{array}{c} \rho \mathbf{u} \\ \rho \mathbf{u}\otimes \mathbf{u} + P \mathbf{I} \\ \mathbf{u} ( E + P )
 \end{array} 
 \right) = 
 \left( \begin{array}{c} 0 \\ 0 \\ 0 \end{array} \right),
\end{equation}
where $\rho$ denotes the mass density, $\mathbf{u}=(u,v)$ the velocity vector, $P$ the fluid pressure, $E$ the total energy and $\mathbf{I}$ the $2 \times 2$ identity matrix. 
 $\mathbf{u} \otimes \mathbf{u}$ is the dyadic product of the velocity vector with itself.
The system is closed using a perfect gas law (the equation of state (EOS)) $$P = (\gamma-1)\left( E - \frac{1}{2}\rho \mathbf{u}^2 \right)$$, with $\gamma$ is the ratio of specific heats.
The sound speed is defined as $c=\sqrt{\gamma P/\rho}$ and the internal energy as $e= E - \frac{1}{2}\rho \mathbf{u}^2$.
Physically admissible states
are the states such that $\rho>0$ and $P>0$.\\
A general formulation of this nonlinear system of hyperbolic 
conservation laws is given by
\begin{equation} \label{eqn.pde.nc} 
  \frac{\partial \U}{\partial t} + \nabla \cdot \tens{\F}(\U)  = \bm{0} , \qquad \xx \in \Omega \subset \mathbb{R}^2, \; t \in \mathbb{R}_0^+, 
\end{equation} 
with appropriate initial and boundary conditions
where $\xx=(x,y)$ is the coordinate vector, $\U=(\rho, \rho u, \rho v, E)$ is the vector of $4$ conserved variables, 
$\tens{\F} = (\mathbf{f}_1, \mathbf{f}_2)$ is the conservative nonlinear flux tensor depending on $\U$.
%
%  R E S I D U A L      D I S T R I B U T I O N     S C H E M E S
%
\section{Residual distribution schemes}  \label{sec:RD}


\subsection{Basics} 
The computational domain $\Omega$ is discretized with $N_e$ conformal non-overlapping elements with characteristic length $h$, the set of all
the elements is denoted by ${\Omega}_h$, 
the list of degrees of freedom (DoFs) is denoted by $\Sigma_h$, 
and the total number of DoFs in one cell is $N_{DoF}$. 
The generic element is called $K$ and the volume of a cell $|K|$, which is for 1D the length of the cell, while in 2D the area. 
For every vertex index $\sigma$ we define $K_{\sigma}$ the subset of elements containing $\sigma$ as a node
\begin{equation*}
K_{\sigma} = \bigcup_{K\in {\Omega}_h | \sigma \in K} K.
\end{equation*}
We denote by $S_{\sigma}$ the standard median dual cell obtained by joining the gravity centres of the elements in $K_\sigma$ with the mid-points of the edges emanating from $\sigma$ whose area is given by
\begin{equation}\label{S_sigma}
|S_\sigma|=\frac{1}{N_{DoF}}\sum_{K, \sigma \in K} |K|.\,
\end{equation}
 see figure~\ref{fig:notation} for an illustration.
We denote by $\mathcal{V}_K$ the set of all neighbour cells and $\mathcal{W}_K$ the 
set of neighbour cells sharing one edge.
The time domain $[0,T]$ is approximated by a set of time intervals $[t_n,\,t_{n+1}]$ and we denote
by $\Delta t =t_{n+1}-t_n$ the time step. \\

Following the Galerkin finite element method (FEM), the solution approximation space
$V_h$ is given by globally continuous polynomials of degree $k$:
\begin{equation}\label{eq:Vh}
V_h= \left\{ \U \in L^2(\Omega_h) \cap C^0(\Omega_h), \; \; \U_{|K} \in \mathbb{P}^k, \; \; \forall K \in \Omega_h  \right\}
\end{equation}
The numerical solution $\U_h^n \simeq \U(\xx,t^n)$ is represented on each element by a linear combination of shape functions 
$\varphi_\sigma \in V_h$
which are assumed to be continuous within the elements and on the faces of the elements
\begin{equation} \label{approx_uh}
  \U_h^n(\xx) = \sum_{\sigma \in \Omega_h}  \U_\sigma^n \, \varphi_\sigma(\xx) , 
  \quad \xx \in \Omega,
\end{equation}
with coefficients $\U_\sigma^n$ to be determined by a numerical method. 
In this work we employ Bernstein basis functions $\left\{ \varphi_{\sigma_h} \right\}_{\sigma_h}$ of order $k$. 

 The drawback of using Bernstein polynomials is that not all degrees of freedom $\U_{\sigma}^n$ in the expansion \eqref{approx_uh} will represent the solution values at certain nodes, however, the advantage of this family of shape functions is their positivity on $K$ that will enforce, the positivity of the mass matrix, as we shall see in the coming section.

On triangular elements, the expressions for the Bernstein shape functions are given by
\begin{multicols}{2}
\begin{itemize}
	\item Order 1 ('B1'): 
	\begin{equation*}
	\varphi_1 = x_1, \ \varphi_2 = x_2, \ \varphi_3 = x_3. \quad \quad \quad \quad
	\end{equation*}
	
	\item Order 2 ('B2'):
	\begin{align*}
	& \varphi_1 = x_1^2, \ \varphi_2 = x_2^2, \ \varphi_3= x_3^2, \\
	& \varphi_4 = 2 x_1 x_2, \ \varphi_5 = 2 x_2 x_3, \ \varphi_6 = 2 x_1 x_3.
	\end{align*}

	\item Order 3 ('B3'):
	\begin{align*}
	& \varphi_1 = x_1^3, \ \varphi_2 = x_2^3, \ \varphi_3= x_3^3, \\
	& \varphi_4 = 3 x_1^2 x_2, \ \varphi_5 = 3 x_1 x_2^2, \ \varphi_6 = 3 x_2^2 x_3, \\
	& \varphi_7 = 3 x_2 x_3^2, \ \varphi_8 = 3 x_1 x_3^2, \ \varphi_9 = 3 x_1^2 x_3, \\
	& \varphi_{10} = 6 x_1 x_2 x_3.
	\end{align*}
	
\end{itemize}
	
	\begin{figure}[H]
	\centering
\includegraphics[scale=0.3]{./FIG/Triangle_B2.eps}\\
\includegraphics[scale=0.3]{./FIG/Triangle_B3.eps}
\caption{Nomenclature of the DoFs within a $B_2$ (upper triangle) and a $B_3$ (lower triangle) element. }
\label{Bernstein_dof}
\end{figure}
\end{multicols}
Here, the barycentric coordinates are defined by $x_1$, $x_2$, $x_3.$
The location of the degrees of freedom for the third and fourth order are, moreover, shown in Fig.~\ref{Bernstein_dof}. 
%======================================================
% FIG
\begin{figure}
  \begin{center}
    \includegraphics[width=0.75\textwidth]{FIG/notation2.eps}
    \caption{ \label{fig:notation}
      Notation for domain $\Omega_h$, its boundary $\Gamma$, cells, dual cells and associated normals.
    }
  \end{center}
\end{figure}
%===========================================================
% Approx of F(U_h)
The approximation of $\tens{F}(\U_h)$ in cell $K$ can be done in two possible ways, as explained and commented in \cite{AbgrallHO2018}, too. One can either evaluate the values of the flux at the DoFs from the data $U_h$, defining $\tens{\F}(\U_h)$ as:
\begin{equation}
\label{flux:approximation}
\tens{\F}(\U_h^n)\approx \sum_{\sigma\in K}\tens{\F}_\sigma \varphi_\sigma,
\end{equation}
which leads to a quadrature-free implementation since the integrals of the shape functions and/or gradients can be evaluated explicitly. Alternatively, one can define $\tens{\F}(\U_h)$ as the flux evaluated for the local value of $\U_h$ at the quadrature point, since both approaches are formally equivalent from the accuracy point of view. 
 

\subsection{Spatial Residual Distribution scheme}

At the heart of a residual distribution scheme resides the notion of 'residual' on each element
which can be better illustrated considering the simpler steady problem
\begin{equation} \label{eqn.pde} 
  \nabla \cdot \tens{\F}(\U)  = \bm{0} , \qquad \xx \in \Omega \subset \mathbb{R}^2 .
\end{equation} 
The 'total residual' in cell $K\in \Omega_h$ of $\U$ is defined as
\begin{equation} \label{eq:residual}
  \Phi^K \left( \U \right) =   \Int_{K} \nabla \cdot  \F(\U)  \, d\xx = \Int_{\partial K} \F(\U) \cdot \bm{n}  \, ds,
\end{equation}
and the entity called 'fluctuation' or 'residual' on $K$ as the contribution to $\Phi^K$
from a degree of freedom $\sigma$ within element $K$. 
Here to simplify we only consider
degrees of freedom which coincide with the vertices of $K$.
Note that the following conservation property holds true
\begin{equation} \label{eq:fluctuation}
  \Phi^K \left( \U_h \right)  = \Sum_{\sigma \in K} \phi_\sigma^K, \; \forall K\in \Omega_h .
\end{equation}
A RD numerical scheme is entirely determined by the strategy with which one
distributes the the total residual amongst the degrees of freedom $\sigma$ .
This strategy %to distribute the total residual amongst the degrees of freedom $\sigma$ 
in \eqref{eq:fluctuation} is defined by means of distribution coefficients $\beta_\sigma$ as
\begin{equation} \label{eq:beta}
  \phi_\sigma^K = \beta_\sigma \Phi^K ,  \; \forall\sigma \in K .
\end{equation}
Hence one specific RD scheme is defined for each and every set of parameters $\beta_{\sigma}$.
The conservation property \eqref{eq:fluctuation} enforces that
\begin{equation} \label{eq:beta_cons}
  \Sum_{\sigma \in K} \beta_\sigma  = 1 .
\end{equation}
The final RD scheme results from collecting the residuals $\phi_\sigma^K$
from cells surrounding the point associated to the specific DoF $\sigma$, that is
\begin{equation} \label{eq:phicons}
\Sum_{K, \sigma\in K} \phi_\sigma^K = 0, \qquad \forall \sigma \in \Omega_h,
\end{equation}
which allows to compute the unknown coefficients of the polynomial solution 
$\U_\sigma$ in \eqref{approx_uh}. \\
In figure~\ref{fig:RD} we illustrate the three steps of a RD scheme: the Computation of the 
total residual, the Distribution 
amongst the degrees of freedom in the cell, and, at last the Gathering of residuals around the DoF.
%======================================================
% FIG
\begin{figure}
  \begin{center}
    \includegraphics[width=1.0\textwidth]{FIG/RD2.eps}
    \caption{ \label{fig:RD}
      Illustration of the three steps of the residual distribution approach: Compute total residual, Distribute
      them amongst the degrees of freedom and finally Gather them.
    }
  \end{center}
\end{figure}
%===========================================================
In the case the DoF $\sigma$ belongs to the physical boundary $\Gamma$
then \eqref{eq:phicons} can be split into internal and boundary contributions as
\begin{equation} \label{eq:phiconsBC}
  \Sum_{K, \sigma\in K} \phi_\sigma^K + \Sum_{\gamma\in \Gamma, \sigma\in \gamma} \phi_\sigma^\gamma = 0, \qquad \forall \sigma \in \Gamma,
\end{equation}
where $\gamma$ is any edge on the boundary $\Gamma$ of $\Omega_h$. If one assumes
that $\U=g$ on $\Gamma$, then both residuals fulfil
\begin{eqnarray} \label{eq:phiconsBC2}
  \Sum_{\sigma\in K} \phi_\sigma^K &=& \Int_{\partial K} \F( \U_h) \cdot \bm{n} \, ds \qquad \forall K , \\
  \Sum_{\sigma\in \gamma} \phi_\sigma^\gamma &=& \Int_{\gamma} \left( \mathcal{F}_n(\U_h,g)- \F( \U_h) \cdot \bm{n} \right)  \,ds , \qquad \forall \sigma \in \Gamma,
\end{eqnarray}
where $\mathcal{F}_n$ is a numerical flux in the normal direction to boundary edge $\gamma$.

% \subsubsection{Low Diffusion A scheme, N scheme and PSI scheme}
% The LDA scheme of P.~Roe \cite{Roe87} is an upwind scheme which determines 
% one or two node targets depending on the advection direction $\bm{a}$. 
% If a one target node is determined then the residual is entirely assigned
% to the target node, see figure~\ref{fig:onetwo} left panel.
% On the contrary if two target nodes, $i$ and $j$, are determined, 
% see figure~\ref{fig:onetwo} right panel, 
% then the residual is distributed amongst them by defining 
% \bea
% \beta_i^{\text{LDA}} = \frac{|T_{ilk}|}{|T_{ilj}|}, \qquad
% \beta_j^{\text{LDA}} = \frac{|T_{ljk}|}{|T_{ilj}|}, \qquad
% \beta_l^{\text{LDA}} = 0
% \eea
% and
% \bea
% \Phi^K = \Phi_i^K + \Phi_j^K + \Phi_l^K, \qquad 
%  \Phi_k^K = \beta_k^{\text{LDA}} \Phi^{\text{LDA}}, \; \; \text{ for }  k=i,j,l .
% \eea
% From basic trigonometry arguments we deduce that 
% \bea
% \beta_i^{\text{LDA}} = \frac{k_i^+}{ \sum_{p \in K} k_p^+ } \geq 0,
% \eea
% and they do not depend on the solution. Moreover we have $\beta_p^{\text{LDA}}\leq 1$
% for all point $p$ in cell $K$. 

% The N scheme \cite{Roe87} is also an upwind scheme for simplexes.
% The goal is to define an upwind RD scheme that generalizes
% the classical upwind scheme in 1D.
% The total residual is 
% distributed amongst the two target nodes for instance by projecting the advection vector such 
% that $\bm{a}=\bm{a}_i+\bm{a}_j$, see figure~\ref{fig:onetwo} middle panel. 
% It implies that for the upstream node $l$
% one fixes $\beta_l^{\text{N}}=0$, while $\beta_i^{\text{N}} >0$ and $\beta_j^{\text{N}}>0$, are deduced 
% by substituting $\bm{a}$ by $\bm{a}_i+\bm{a}_j$ in the total residual definition, hence
% \bea \label{eq:betaN}
% \Phi^K = \Phi_i^K + \Phi_j^K + \Phi_l^K, \qquad 
%  \Phi_k^K \equiv \Phi_k^K(\bm{a}_k) = \beta_k^{\text{N}} \Phi^K, \; \; \text{ for }  k=i,j,l
% \eea

% The PSI scheme of R.~Struijs \cite{Struijs93} is often refered to as the 'limited N' scheme
% because the coefficients $\beta$ are constructed by taking only the positive part of 
% those of the N scheme as
% \bea
% \beta_i^{\text{PSI}} = \frac{ (\beta_i^{\text{N}})^+}{ \Sum_{j\in K} (\beta_j^{\text{N}})^+}, 
% \eea
% for all point $i$ of $K$,
% where $\beta_i^{\text{N}}$ are the coefficients of the N scheme obtained from (\ref{eq:betaN}).
% Immediately it follows that: $\beta_i^{\text{PSI}}\geq 0$ for all $i$ 
% and $\Sum_{i \in K} \beta_i^{\text{PSI}} = 1$.


%\subsubsection{Streamline Upwind Petrov Galerkin (SUPG)} \label{ssec:SUPG}
%The SUPG scheme proposed by Hughes in \cite{hughes86} can be recast into the residual form
%\begin{equation} \label{eq:phiSUPG}
%  \phi_\sigma^K(\U_h)  =  \Int_{\partial K} \varphi_\sigma \F(\U_h)\cdot \bm{n} \, ds - \Int_{K} \nabla\varphi_\sigma \cdot \F(\U_h)  \, d\xx
%            + h_K \Int_{K} \left( \nabla_{\U}\F(\U_h)\cdot\nabla\varphi_\sigma  \right) 
%                     \tau \left( \nabla_{\U}\F(\U_h)\cdot\nabla\U_h           \right) \,d\xx,
%\end{equation}
%with $\tau>0$ and $h_K$ is the characteristics length of cell $K$.
%Then once $\phi_\sigma^K$ are determined for each DoF $\sigma$, 
%then $\Phi_K$ can be computed from (\ref{eq:residual}) and $\beta_K$ from (\ref{eq:beta}).
%Conservation property (\ref{eq:phicons}) is ensured by construction.
%

%\subsubsection{Galerkin FEM with Jump stabilization (GJ)} \label{ssec:GalerkinJump}

%The so-called Galerkin FEM with jump stabilization RD scheme seen in Burman \cite{burman04} consists in 
%considering residuals of the form
%\begin{equation} \label{eq:phiGJ}
%  \phi_\sigma^K(\U_h)  =  \Int_{\partial K} \varphi_\sigma \F(\U_h)\cdot \bm{n} \, ds - \Int_{K} \nabla\varphi_\sigma \cdot \F(\U_h)  \, d\xx
%                      + \Sum_{e \in \partial K} \theta h_e^2 \Int_{e} \left[ \nabla \U_h \right] \cdot \left[ \nabla\varphi_\sigma \right]  \,ds,
%\end{equation}
%where $\theta\geq 0$ and we denote $\left[ \nabla \psi \right] = \nabla \psi|_K - \nabla \psi |_{K'}$ where $e=K \cap K'$
%for any function $\psi$. $\beta_K$ are deduced mimicking the procedure described for SUPG scheme.
%

%
%\subsubsection{Local Lax-Friedrichs (LxF)} \label{ssec:LxF}
%A local Lax-Friedrichs type nodal residual is defined by
%\begin{equation} \label{eq:phiLxF}
%  \phi_\sigma^K(\U_h)  =  \Int_{\partial K} \varphi_\sigma \F(\U_h)\cdot \bm{n} \, ds - \Int_{K} \nabla\varphi_\sigma \cdot \F(\U_h)  d\xx
%                      + \alpha_K ( \U_h - \overline\U_h ),
%\end{equation}
%where $\overline\U_h$ is the arithmetic average of all degrees of freedom defining $\U_h$ in $K$.
%The viscosity coefficient $\alpha_K$ is connected to the spectral radius of the normal flux Jacobian matrix
%$\bm{A}(\U)=\nabla_{\U} \F (\U)\cdot \bm{n}$.
% system (\ref{eqn.pde.nc}) can be formally integrated on $[t^n, t^{n+1}]$ as
%\begin{equation}\label{eq:rhoS}
%\rho_S \equiv \rho_S( \bm{A}(\U) ) = \max ( |\lambda_1|, \ldots , |\lambda_m| ),
%\end{equation}
%as
%%\label{eq:alphaK}
%$\alpha_K = N_K \max_{\sigma \in K} \left( \rho_S(\nabla_{\U} \F (\U)\cdot \nabla \varphi_\sigma \right)$,
%where $N_K$ is the number of dof in the cell $K$.
%$\beta_K$ are deduced mimicking the procedure described for SUPG scheme.
%
%
%\subsubsection{Limited residual distribution scheme (RDS)} \label{ssec:LxF}
%Another example is the Limited residual distribution scheme (RDS) of Abgrall \textit{et al.} \cite{}
%for which there does not exist a straightforward variational formulation
%\begin{equation} \label{eq:phiRDS}
%  \phi_\sigma^K(\U_h)  =  \beta_{\sigma}^K \Int_{\partial K}  \F(\U_h)\cdot \bm{n} \, ds  
%    + h_K \Int_K \left( \nabla_{\U}\F(\U_h)\cdot\nabla\varphi_\sigma  \right) 
%                     \tau \left( \nabla_{\U}\F(\U_h)\cdot\nabla\U_h           \right) \,d\xx,
%\end{equation}
%or
%\begin{equation} \label{eq:phiRDS2}
%  \phi_\sigma^K(\U_h)  =  \beta_{\sigma}^K \Int_{\partial K}  \F(\U_h)\cdot \bm{n} \, ds  
%    + \Sum_{e \in \partial K} \theta h_e^2 \Int_{e} \left[ \nabla \U_h \right] \cdot \left[ \nabla\varphi_\sigma \right]  \,ds,
%\end{equation}
%where $\beta_{\sigma}^K$ are parameters that guarantee the conservation and such that $\Sum_{\sigma \in K} \beta_{\sigma}^K = 1$.
%$\beta_K$ are deduced mimicking the procedure described for SUPG scheme.
%



\subsection{Time Residual Distribution scheme via a deferred correction-like method} \label{ssec.TimeRD}
In this section we recall the construction of the high-order accurate time discretisation for residual distribution schemes presented in \cite{Abgrall2017,AbgrallHO2018}.
Starting by considering the numerical solution at a discrete time $t^n$ denoted by $\U^n$, we search for the 
solution at $t^{n+1}$ denoted by $\U^{n+1}$.
We split each interval $[t^n, t^{n+1}]$ into sub-timesteps 
$t^n\equiv t^{n,0} < t^{n,1} < \ldots < t^{n,m} < \ldots < t^{n,M} \equiv t^{n+1}$.
For the $m$-th subinterval $[t^{n,m},t^{n,m+1}]$, we introduce the correction indices
$r= 0, \ldots, R$ and further denote the solution at correction index $r$ of the sub-timestep $m$ 
by $\U^{n,m,r}$. In addition we denote the solution vector of the $r$-th corrections by
 system \eqref{eqn.pde.nc} can be formally integrated on $[t^n, t^{n+1}]$ as
\begin{equation}\label{eq:Ucorr}
\U^{(r)} = \left( \U^{n,0,r}, \ldots, \U^{n,M,r}  \right).
\end{equation} 
The timestepping approach is similar but not identical to the deferred correction methodology of \cite{dutt2000,Minion2,shu-dec} and 
one proceeds  within the time step $[t^n, t^{n+1}]$ as follows:
\begin{enumerate}
\item We initialize for $m=1,\ldots, M$: $ \U^{n,m,0} =  \U^n$;
\item for each correction $r=0,\ldots,R-1$, we iterate for $m=1,\ldots, M$, such that,\\
knowing $\U^{n,m,r}$, we evaluate $\U^{n,m,r+1}$ as the solution of 
\begin{equation}\label{eq:defcor}
\mathcal{L}^1(\U^{n,m,r+1})=\mathcal{L}^1(\U^{n,m,r})-\mathcal{L}^2(\U^{n,m,r})
\end{equation}
\item set $\U^{n+1}=\U^{n,M,R}.$
\end{enumerate}

In \cite{Abgrall2017} it has been proved that, under some assumption on the differential operators
$\mathcal{L}_\Delta^1,\mathcal{L}_\Delta^2$ depending on a parameter $\Delta$, the deferred correction-like method is convergent, and after $R$ iterations
the error is smaller than $\nu^R||\U^{(0)}-\U_{\Delta}^{\star}||$, where $\nu=\frac{\alpha_2}{\alpha_1} \Delta <1$ 
is a real constant depending on the operators $\mathcal{L}_\Delta^1,\mathcal{L}_\Delta^2$.\\
The $\alpha_1$ and $\alpha_2$ are assumed to be the parameters of the operators such that
$\mathcal{L}_\Delta^2$ has a unique root $\U_\Delta^\star$ (such that $\mathcal{L}_\Delta^2(\U_\Delta^\star)=0$), 
$\mathcal{L}_\Delta^1$ is coercive with coercivity constant $\alpha_1$, 
and $\mathcal{L}_\Delta^2-\mathcal{L}_\Delta^1$ is uniformly Lipschitz continuous with Lipschitz constant $\alpha_2 \Delta$. 

Let us first recall the low order differential operator $\mathcal{L}^1$ then 
the high order differential operator $\mathcal{L}^2$.
To do so the starting point consists in recalling that
 system \eqref{eqn.pde.nc} can be formally integrated on $[t^n, t^{n+1}]$ as
\begin{equation}
\U(\xx,t^{n+1}) = \U(\xx,t^{n}) + \Int_{t^n}^{t^{n+1}} \nabla\cdot \tens{F}( \U (x,t) ) \, dt,
\end{equation}
and the solution be approximated with a quadrature rule
\begin{equation}
\U(\xx,t^{n+1}) \simeq \U(\xx,t^{n}) + \Delta t \Sum_{l=0}^r \omega_l \, \nabla\cdot \tens{F}( \U (x,t_l) ).
\end{equation}

\subsubsection{Low Order Differential Operator $\mathcal{L}^1$}
For any $\sigma \in K$, we define $\mathcal{L}^1$ as
\begin{equation}\label{eq:L1}
\mathcal{L}^1_\sigma ( \U^{(r)} ) =\mathcal{L}^1_\sigma ( \U^{n,1,r}, \ldots , \U^{n,M,r})
\end{equation}
where in particular we have for a generic sub-timestep $m$ at a correction $r$ that
\begin{equation}
\mathcal{L}^1_\sigma (\U^{n,m,r})=|C_\sigma| \left(  \U_\sigma^{n,m,r} - \U_\sigma^{n,0,r} \right) + \Sum_{K | \sigma\in K} \Int_{t^{n,0}}^{t^{n,m}} \mathcal{I}_0 \left( \phi_\sigma^K(\U^{(r)}) ,t\right)\,dt, 
\end{equation}

where $\mathcal{I}_0$ represents any first order piecewise-constant interpolant under the following notation
\begin{equation}
 \phi_\sigma^K(\U^{(r)}) = \phi_\sigma^K(\U^{n,1,r}),  \ldots , \phi_\sigma^K(\U^{n,M,r}).
\end{equation} 
As it stands, system \eqref{eq:L1} is a time implicit system. An explicit in time version is
obtained by considering $\mathcal{I}_0$ as being a simple approximation of $\U^{n,0}$ for all $m$, so that \eqref{eq:L1} becomes
\begin{equation}\label{eq:L1b}
\mathcal{L}^1_\sigma (\U^{n,m,r})=
|C_\sigma| \left(  \U_\sigma^{n,m,r} - \U_\sigma^{n,0,r} \right) + \Delta t \, \xi_m \, \Sum_{K | \sigma\in K} \phi_\sigma^K(\U^{(0)})  
\end{equation}
with $\xi_m$ satisfying for $m=1,\ldots,M$  $t_{n,m}=t_n+\xi_m \Delta t$ and $0=\xi_0<\ldots<\xi_m<\xi_{m+1}<\ldots \xi_M=1$ within the considered time interval $[t_n, t_{n+1}]$.\\
The coefficients $|C_\sigma|$ play the role of the dual cell measure and and in order for (\ref{eq:L1}) to be solvable we have to satisfy the constraint
\begin{equation}\label{Csigma_mood}
|C_\sigma| = \Int_K \varphi_\sigma( \xx) \, d\xx >0,
\end{equation}
This requirement has a direct consequence on the choice of the polynomial basis $\left\{ \varphi_\sigma \right\}_\sigma$. 
For instance, the classical Lagrange basis on simplex is disqualified as it does not verify \eqref{Csigma_mood} for $k>1$, and this is the reason why we consider Bernstein polynomials \cite{Bernstein1912,Lorentz_book_Bersntein53} for high order approximations. Indeed, Bernstein basis functions verify $\varphi_\sigma(\xx)\geq 0$ for all $\sigma$ and $\xx$, and $\Sum_{\sigma} \varphi_\sigma(\xx)=1$
for all $\xx$, and it is easy to deduce that \eqref{Csigma_mood} is fulfilled. \\
The low order differential operator $\mathcal{L}^1_\sigma$ constructed this way is then of high accuracy in space and explicit in time.


\subsubsection{High Order Differential Operator $\mathcal{L}^2$}
The high order differential operator $\mathcal{L}^2_\sigma$ for a generic sub-timestep $m$ at a correction $r$ is defined as
\begin{equation}\label{eq:L2}
\mathcal{L}^2_\sigma ( \U^{n,m,r} ) =
\Sum_{K | \sigma\in K} \left( 
\Int_K \varphi_\sigma ( \U^{n,m,r} - \U^{n,0,r}) \, d\xx +  \Int_{t^{n,0}}^{t^{n,m}} \mathcal{I}_M \left( \phi_\sigma^K(\U^{(r)}) ,s\right)\,ds   \right)  
\end{equation}
Once the coefficients of the interpolating polynomial $\mathcal{I}_M$ of degree $M$ are computed, we perform
the exact integration to obtain the approximation for every row of \eqref{eq:L2} in the form
\begin{equation}
 \Int_{t^{n,0}}^{t^{n,m}} \mathcal{I}_M \left( \phi_\sigma^K(\U^{n,0,r}),\ldots , \phi_\sigma^K(\U^{n,M,r}) ,s \right)\,ds 
=  \Sum_{l=0}^M \zeta_{l,m}  \phi_\sigma^K(\U^{n,l,r}) ,
\end{equation}
where $\zeta_{l,  m}$ are approximation coefficients.
The high order differential operator $\mathcal{L}^2$ ensures a high order approximation
of the space-time term $\partial_t \U + \nabla \cdot \tens{F}(\U)$. 
Unfortunately, as it stands, the operator is implicit in time. 
Therefore to turn it into an explicit one,
the iterative time-stepping 
formulation depicted in the algorithm \eqref{eq:defcor} is re-employed.

\begin{remark}
As a matter of completeness, one should note that both \eqref{eq:L1} and \eqref{eq:L2} make use of  residuals $\phi^K_\sigma( \U^{n,m,r} )$ for all $\sigma \in K$, and all $K$, which are computed via any spatial residual distribution scheme as seen in the previous sections, and where the boundary conditions are applied within the residual computation. More details on the actual spatial discretization scheme will be specified in the forthcoming sections, as it is part of the main idea behind this work.
\end{remark}

==> intro.tex <==

% ======== INTRODUCTION ===================
\section{Introduction} \label{sec:introduction}
 
In gas dynamics, a highly investigated topic is given by flows displaying strongly interacting discontinuities. To approximate this physics, several models exist. The Euler equations in multi-dimensions, count among this models, and one of its main features is to be a hyperbolic system, and as such, it allows to represent physical behaviours such as rarefactions, contact discontinuities and shocks. Even though uncountable typologies of different approximation strategies exist to tackle the solution to this problem, each method designed so far encounters some restrictions such as providing a highly accurate approximation guaranteeing the robustness of the considered method, i.e. the capability to provide a solution even in case of extremely tough initial conditions. Methods with this two features need, moreover, to face the requirement of not being excessively expensive, both in terms of computational time and memory related issues. Indeed, to explain what is meant, we do have a vicious cycle, as an accurate method might affect negatively the robustness and computational efficiency, while on the other hand, a robust and efficient approach might decrease the accuracy and, finally, an efficient one, is often impacting negatively on both the accuracy and robustness.
The proposed methodology, based on Residual Distribution schemes, represents a good compromise between this three requirements, as it is designed for high order accuracy and guarantees at the same time an overall excellent robustness. The efficiency of the method is not accounted in the present work, but, in general, due to its characterising traits, Residual Distribution schemes can be rewritten in a parallelized form, as the way they are constructed allows to split for computation, for example, the domain, in several parts easily.  This allows for an efficient computational time cost management. As for the memory efficiency, the design principle of this class of schemes guarantees a compact approximation stencil even for high order of accuracy, which would also hold for example for Discontinuous Galerkin (DG) methods, but not, for example, for Finite Volume methods. In \cite{enordhigh, Cangiani2013, AbgrallViville2017} it has been shown how Residual Distribution schemes allow also, furthermore, to consider overall less nodes w.r.t. DG methods.\\

Although the construction of first-order, robust and stable Residual Distribution (RD) schemes has been achieved in the 80s, the construction of  very high accurate and robust RD schemes for unsteady problems is more recent (see \cite{Abgrall2010,AbgrallENUMATH2015,Abgrall2017,AbgrallHO2018}). 
Within this paper, we consider a RD formulation based on a finite element approximation of the solution as a globally continuous piecewise polynomial.
Further, we follow \cite{AbgrallENUMATH2015,Abgrall2017}, where we have shown how one can solve a scalar version of a hyperbolic system with a method that approximates the spatial term using a RD approach, without having to solve a large linear system with a sparse mass matrix and its extension to systems achieved within the work in \cite{AbgrallHO2018}. This reformulation allows to avoid any mass matrix "inversion" while solving an explicit scheme. This is achieved by first approximating the time operator in a consistent way with the spatial term. A priori, this would lead either to an implicit method in case of a nonlinear approximation, as done in order to avoid spurious oscillations in the case of discontinuous solutions, or at minima the inversion of a sparse but non diagonal matrix.  This apparent difficulty can be solved by applying a Deferred Correction-like time-stepping method (\cite{Abgrall2017,AbgrallHO2018}) inspired by \cite{shu-dec,Minion2} among others, but recast in a different way, and the use of proper basis functions. It has been demonstrated in \cite{AbgrallENUMATH2015,Abgrall2017} that Bernstein polynomials are a suitable choice, but this is not the only possible one. The idea to use as shape functions the Bernstein polynomials, instead of the more typical Lagrange polynomials, has been discussed in \cite{Abgrall2010, Abgrall2017} applied to the context of high order Residual Distribution schemes.\\


The essence of the present chapter is to apply to the high order explicit Residual Distribution approach, presented in Chapter \ref{ch:HOpaper}, a blending, which is designed as an ``a posteriori'' limiter, in order to ensure a highly accurate representation of the solution in the areas of smooth flows, while ensuring a non-oscillatory behaviour across strong interacting discontinuities. The main features of the designed scheme should also ensure the overall robustness and allow for a \textit{fail-safe} numerical solution, in order to provide for any studied condition a physically meaningful approximated solution.\\
The proposed ``a posteriori'' limiting strategy is obtained via a Multidimensional Optimal Order Detection (MOOD) Method by considering a candidate solution for the next time iteration given by a non-dissipative scheme for the spatial terms, such as the standard Galerkin method, which is characterized by highly accurate approximations in smooth regions of the flow, but is not robust and displays numerical oscillations in case of strong interacting discontinuities. The ``a posteriori'' limiting detects then the cells which display any physically non admissible solutions and those cells are \textit{locally} re-approximated by discarding the candidate solution and recomputing the solution via a more dissipating spatial numerical scheme.\\

In literature, the MOOD approach has first emerged in a Finite Volume context (\hspace{1sp}\cite{Clain2011,Diot2012,Diot2013}), with the main idea to approximate solutions via high order polynomial reconstruction and in case the detecting criteria evidence any troubled cell, the polynomial degree in the associated cell is decremented, and the solution is locally recomputed.
In a second approach, the MOOD strategy has been extended to the Finite Element discontinuous Galerkin schemes (\hspace{1sp}\cite{Dumbser2014,Dumbser2016}), where the leading idea has been to apply unlimited discontinuous Galerkin schemes with a high approximation degree for a candidate solution, and, detected troubled cells are re-evaluated by discarding the candidate solution. In those cells, sub-cells are introduced and a more robust second order total variation diminishing (TVD) finite volume scheme is applied to update to the next time-step the sub-cell averages within the troubled DG cells. The new sub-grid data at the next time level are then gathered back into a valid cell-centred DG polynomial of degree N by using a classical conservative and higher order accurate finite volume reconstruction technique.
Recently,  in \cite{Vilar2018}, a further method similar to this last one has been proposed, where the DG reconstructed flux on the sub-cell boundaries is substituted locally, in case the detection criteria are activated, by a robust first-order or second-order TVD numerical flux.\\

The idea of the proposed method, while certainly inspired by these previous works, is, nevertheless on a different level. The main difference, indeed, is given by two different traits, as for instance, the novel methodology consists in the re-computation of the local troubled cell by taking the very same element typology, i.e. the polynomial degree of the considered shape functions is kept the same, and, moreover, the cell is recomputed at a global level, in the sense that we do not recompute the sub-cell values via a different approach, but simply compute the whole cell with a more dissipating scheme, and by the Lax-Wendroff theorem, we have by construction the guarantee of conservation.\\
Concerning the detection criteria itself, we have, furthermore investigated two different approaches within this work: the first one  based on \cite{Clain2011,Diot2012,Diot2013,Dumbser2016}, while the second has been taken after \cite{Vilar2018}.\\

To this end, this chapter has been organized as follows. 
In Section \ref{sec:Euler} we present briefly the considered model equations and in Section \ref{sec:RD} we recall the overall framework of the considered discretizations techniques. First, we recall the basics of the RD schemes, where, in particular we summarize the leading traits of this approach for the steady case along its extension to the unsteady case for high order of accuracy as in \cite{AbgrallHO2018}. Section \ref{sec:MOOD} describes the generic idea of the ``a posteriori'' Multidimensional Optimal Order Detection Method. In this section we describe the detailed detection procedure, along with the two different considered detection strategies inspired by \cite{Clain2011} and \cite{Vilar2018}. Finally we provide in Section \ref{sec:numerics} several numerical benchmark problems, both in one- and two-dimensions to assess the accuracy and overall robustness of the proposed methodology and to investigate the major differences given by the two different detection criteria. Last, in the final section, we provide some conclusive remarks along with the perspectives of this work.
This work follows strictly \cite{BacigaluppiMood2018}, currently in preparation for submission.
